Charge-Density-Wave Oscillator Networks for Solving Combinatorial Optimization Problems

Many combinatorial optimization problems fall into the non-polynomial time NP-hard complexity class, characterized by computational demands that increase exponentially with the size of the problem in the worst case. Solving large-scale combinatorial optimization problems efficiently requires novel hardware solutions beyond the conventional von Neumann architecture. We propose an approach for solving a type of NP-hard problem based on coupled oscillator networks implemented with charge-density-wave condensate devices. Our prototype hardware, based on the 1T polymorph of TaS2, reveals the switching between the charge-density-wave electron-phonon condensate phases, enabling room-temperature operation of the network. The oscillator operation relies on hysteresis in current-voltage characteristics and bistability triggered by applied electrical bias. This work presents a network of injection-locked, coupled oscillators whose phase dynamics follow the Kuramoto model and demonstrates that such coupled quantum oscillators naturally evolve to a ground state capable of solving combinatorial optimization problems. The coupled oscillators based on charge-density-wave condensate phases can efficiently solve NP-hard Max-Cut benchmark problems, offering advantages over other leading oscillator-based approaches. The nature of the transitions between the charge-density-wave phases, distinctively different from resistive switching, creates the potential for low-power operation and compatibility with conventional Si technology.

==> preamble.tex <==
% This file defines the handy packages, notations, commands for .tex file
% To use this file, put this file in the same directory as the main .tex file, and add \input{preamble.tex} at the beginning
% Check LatexTemplate.tex for example illustrations

%%\usepackage[letterpaper, margin=1in]{geometry}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{xcolor}
% \usepackage{appendix}
\usepackage{comment}
\usepackage{balance}


%-------------------------------------------- Packages for displaying Image------------------------------------------
\usepackage{graphicx}
\usepackage{subfig}
% \ifCLASSOPTIONcompsoc
% \usepackage[caption=false,font=footnotesize,labelfont=sf,textfont=sf]{subfig}
% \else
% \usepackage[caption=false,font=footnotesize]{subfig}
% \fi
\graphicspath{ {images/}}
% \usepackage{caption}
%--------------------------------------------------------------------------------------------------------------------

%----------------------------------------- Packages for Special Characters ------------------------------------------
\usepackage{pifont}
%--------------------------------------------------------------------------------------------------------------------

%%---------------------------------------------- Packages for Hyperlink ----------------------------------------------
 \usepackage{hyperref}
\hypersetup{
		colorlinks,
		 linkcolor={red!50!black},
		 citecolor={blue!50!black},
		 urlcolor={blue!80!black}
	}
% \usepackage[colorlinks,urlcolor=blue,linkcolor=blue,citecolor=blue]{hyperref} 
%
%\makeatletter
%\let\NAT@parse\undefined
%\makeatother
%\usepackage[colorlinks,urlcolor=blue,linkcolor=blue,citecolor=blue]{hyperref}
%%--------------------------------------------------------------------------------------------------------------------

%---------------------------------------------- Packages for Algorithm-----------------------------------------------
%\usepackage[ruled, vlined]{algorithm2e}
%\usepackage{algorithm2e}
\usepackage{algorithmic}

%--------------------------------------------------------------------------------------------------------------------

%------------------------------------------ Package for String Operation --------------------------------------------
% I use the \IfStrEq command to judge if the input is number ''1''.
\usepackage{xstring}
%--------------------------------------------------------------------------------------------------------------------

%%---------------------------------------------- Packages for Citations-----------------------------------------------
%\usepackage{cite}
%\usepackage[numbers]{natbib}
%\bibliographystyle{apalike} % Author+Year
%% If encounter issue "natbib Error: Bibliography not compatible with author-year citations", delete .aux and .bbl 
%% file and recompile.
%%--------------------------------------------------------------------------------------------------------------------

%%------------------------------------------ Packages for Bibliographic Entries --------------------------------------
%% Put what the text shows up in the reference list into the text
%\usepackage{bibentry}
%\nobibliography*
%%--------------------------------------------------------------------------------------------------------------------

%------------------------------------------------ Packages for Tables------------------------------------------------
\usepackage{multirow}
\usepackage{calc}
\usepackage{adjustbox}
\usepackage{booktabs}

% By default, in the table, the content in the cell tend to move up a little rather than stay in the middle, \mytabspace command can correct his
% This command will not change the row height, but only move the cell content.
% This command can only be applied to a specific cell
\newcommand{\mytabspace}[1]{%
	\parbox[c][\totalheightof{#1}+1\fboxsep+1\fboxrule][c]{\widthof{#1}}{#1}%
}

% Commands used to ENLARGE the top and bottom margin of an entire row, and the row height will increase accordingly
\newcommand\Tstrut{\rule{0pt}{3ex}}       
% "top" strut; Change the last variable to adjust the top margin of a row in the table
\newcommand\Bstrut{\rule[-1.5ex]{0pt}{0pt}} 
% "bottom" strut; Change the first variable to adjust the bottom margin of a row in the table, less frequently used.
\newcommand{\TBstrut}{\Tstrut\Bstrut} % top&bottom struts

\newcommand{\cellvcenter}[1]{\begin{tabular}{l} #1 \end{tabular}}
\usepackage{makecell}
%--------------------------------------------------------------------------------------------------------------------

%----------------------------- Packages for Theorems and Function -----------------------------------------

\usepackage{bbm}
\theoremstyle{plain}
\newtheorem{setup}{Setup}
\newtheorem{fact}{Fact}
\renewcommand*{\thesetup}{S\arabic{setup}}
\newtheorem{problem}{Problem}
\renewcommand*{\theproblem}{P\arabic{problem}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
% \renewcommand*{\theassumption}{A\arabic{assumption}}

%\newtheorem*{definition*}{Definition}
%\newtheorem*{assumption*}{Assumption}
%\newtheorem*{problem*}{Problem}
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem*{corollary*}{Corollary}
%\newtheorem*{proposition*}{Proposition}
%\newtheorem*{remark*}{Remark}
%
%% The following defines command that can customize theorem labelling
%\newtheorem{innercustomgeneric}{\customgenericname}
%\providecommand{\customgenericname}{}
%\newcommand{\newcustomtheorem}[2]{%
	%	\newenvironment{#1}[1]
	%	{%
		%		\renewcommand\customgenericname{#2}%
		%		\renewcommand\theinnercustomgeneric{##1}%
		%		\innercustomgeneric
		%	}
	%	{\endinnercustomgeneric}
	%}
%\newcustomtheorem{customtheorem}{Theorem}
%\newcustomtheorem{customlemma}{Lemma}
%\newcustomtheorem{customproposition}{Proposition}
%--------------------------------------------------------------------------------------------------------------------

%------------------------------ Package for Changing the Bullet Style of Enumerate ----------------------------------
\let\labelindent\relax
\usepackage{enumitem}
%\begin{enumerate}[label=(\roman*)]
%\item
%\end{enumerate}
%--------------------------------------------------------------------------------------------------------------------

%------------------------- Command for Allowing Align Environment to Break Between Pages ----------------------------
\allowdisplaybreaks
%\begin{align*}
%a\\
%b\\
%c\\
%d\\
%e\stepcounter{equation}\tag{\theequation}\label{eq_76}\\
%f\\
%g\\
%h\\
%i
%\end{align*}


%-------------------------------------------- Commands for Letters----------------------------------------
\input{preambleLettersDef.tex}
%--------------------------------------------------------------------------------------------------------------------



%------------------------------------------------- Common Math Operator ---------------------------------------------
\newcommand{\norm}[1]{\|{#1} \|}
\newcommand{\normauto}[1]{\left\|{#1} \right\|}
\newcommand{\normbig}[1]{\big\| #1 \big\|}
\newcommand{\normBig}[1]{\Big\| #1 \Big\|}
\newcommand{\normbigg}[1]{\bigg\| #1 \bigg\|}
\newcommand{\normBigg}[1]{\Bigg\| #1 \Bigg\|}
\newcommand{\crlbkt}[1]{\{ #1 \}}
\newcommand{\crlbktauto}[1]{\left\{ #1 \right\}}
\newcommand{\crlbktbig}[1]{\bigl\{ #1 \bigr\}}
\newcommand{\crlbktBig}[1]{\Bigl\{ #1 \Bigr\}}
\newcommand{\crlbktbigg}[1]{\biggl\{ #1 \biggr\}}
\newcommand{\crlbktBigg}[1]{\Biggl\{ #1 \Biggr\}}
\newcommand{\sqbkt}[1]{[ #1 ]}
\newcommand{\sqbktauto}[1]{\left[ #1 \right]}
\newcommand{\sqbktbig}[1]{\bigl[ #1 \bigr]}
\newcommand{\sqbktBig}[1]{\Bigl[ #1 \Bigr]}
\newcommand{\sqbktbigg}[1]{\biggl[ #1 \biggr]}
\newcommand{\sqbktBigg}[1]{\Biggl[ #1 \Biggr]}
\newcommand{\prnthauto}[1]{\left( #1 \right)}
\newcommand{\prnthbig}[1]{\bigl( #1 \bigr)}
\newcommand{\prnthBig}[1]{\Bigl( #1 \Bigr)}
\newcommand{\prnthbigg}[1]{\biggl( #1 \biggr)}
\newcommand{\prnthBigg}[1]{\Biggl( #1 \Biggr)}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
% \newcommand{\indicator}{\mathbbm{1}}
\newcommand{\indicator}[1]{\mathbf{1}_{\crlbktauto{#1}}}

\newcommand{\st}{\textup{subject to}}
\newcommand{\mxz}{\textup{maximize}}
\newcommand{\mnz}{\textup{minimize}}

\newcommand{\wht}[1]{\widehat{#1}}		% Widehat
\newcommand{\wtd}[1]{\widetilde{#1}}	% Widetilde

\newcommand{\R}{\mathbb{R}}				% Real line R
\newcommand{\NaturalNum}{\mathbb{N}}				% Real line R
\newcommand{\dm}[2]
{
	\IfStrEq{#2}{1}{\R^{#1}}{\R^{#1 \x #2}}
}

\newcommand{\N}{\mathcal{N}}			% Normal Distribution N
\newcommand{\onevec}{\mathbf{1}} 		% Bold 1, All 1 vector

\newcommand{\rank}{\textup{{rank}}} 			% rank
\newcommand{\tr}{\textup{\textbf{tr}}} 			% Trace
\newcommand{\diag}{\textup{\textbf{diag}}} 		% Diag
\newcommand{\cond}{\textup{\textbf{cond}}} 		% Condition number
\newcommand{\vek}{\textup{\textbf{vec}}}			% Vectorization
\newcommand{\expctn}{\mathbb{E}} 	 	% Expectation
\newcommand{\cov}{\textup{\textbf{Cov}}}	 	% Expectation
\newcommand{\CRB}{Cram{\'e}r-Rao bound} % Expectation
\newcommand{\inv}{{-1}} 				% Superscript inverse
\newcommand{\invv}[1]{{\mskip-1mu \scalebox{1.5}[0.75]{-} \mskip-1mu #1}} %
\newcommand{\gotoinf}{\rightarrow \infty} 				% Superscript inverse
\newcommand{\prob}{\mathbb{P}} 				% The upright P to denote probability
\newcommand{\diff}{\textup{d}}				% The d in derivative
\newcommand{\fro}{\textup{F}}			% Subscript for Frobenius norm
\newcommand{\iiddist}{\overset{\textup{i.i.d.}}{\sim}}
\newcommand{\poly}{\textup{poly}}
\newcommand{\polylog}{\textup{polylog}}
\newcommand{\order}[1]{{\cal{O}}(#1)}

% Transpose
\usepackage{amssymb}
\makeatletter
\newcommand*{\T}{{\mathpalette\@transpose{}}}
\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
%\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\top$}}
\makeatother

% The product x sign used in dimension, e.g. R^{m \x n}
% Compared with \times, \x can save more space before and after the operator
\newcommand*{\x}{\mathsf{x}\mskip1mu} 	

% The minus sign
% Compared with -, \m can save more space before and after the operator 
\newcommand*{\minus}{\mathsf{-}\mskip1mu} 

%--------------------------------------------------------------------------------------------------------------------

%---------------------------------------------------- Other Commands ------------------------------------------------
% Allow inline math equation to break at commas
\newcommand{\splitatcommas}[1]{%
	\begingroup
	\begingroup\lccode`~=`, \lowercase{\endgroup
		\edef~{\mathchar\the\mathcode`, \penalty0 \noexpand\hspace{0pt plus .1em}}%
	}\mathcode`,="8000 #1%
	\endgroup
}
% $\splitatcommas{
	%   \frac{1}{2},\frac{3}{5},\frac{8}{13},\frac{21}{34},\frac{55}{89},
	%   \frac{144}{233},\frac{377}{610},\frac{987}{1597},\frac{2584}{4181},
	%   \frac{6765}{10946},\frac{17711}{28657},\frac{46368}{75025},
	%   \frac{121393}{196418},\frac{317811}{514229},\frac{832040}{1346269},
	%   \frac{2178309}{3524578},\frac{5702887}{9227465},
	%   \frac{14930352}{24157817},\frac{39088169}{63245986},\frac{102334155}{165580141}
	% }$

% Allow the equation in itemize or enumerate to align with the item labe
\newcommand\Item[1][]{% 
\ifx\relax#1\relax  \item \else \item[#1] \fi
\abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}

% The following commands are for review responses
% initialize counters for reviewer number and comment number
\newcounter{reviewer}
\setcounter{reviewer}{0}
\newcounter{point}[reviewer]
\setcounter{point}{0}

\makeatletter
\newcommand{\customlabelfig}[2]{%
    \protected@write \@auxout {}{
    \string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}{}}
    }
}
\makeatother

\makeatletter
\newcommand{\customlabelresponse}[2]{%
   \protected@write \@auxout {}{
   \string \newlabel {#1}{{#2}{\thepage}{#2}{#1}{}} 
   }%
   \hypertarget{#1}{#2}
}
\makeatother



% Set the format of reviewer comment numbers and responses.
% \renewcommand{\thepoint}{Q\,\thereviewer.\arabic{point}} 
\renewcommand{\thepoint}{Q\,\arabic{point}} 
\newcommand{\point}[1]{\refstepcounter{point}  \bigskip \medskip \noindent {\fontseries{b}\selectfont \thepoint } \textit{#1}\par}
\newcommand{\reply}{\medskip \noindent \textbf{Reply}:\ }
\newcommand{\reviewerNumber}[1]{\refstepcounter{reviewer}  \bigskip \medskip \noindent \section*{#1} \par}

% Set the format for reviewer headings
\newcommand{\reviewersection}{\stepcounter{reviewer}
                  \section*{Response to Reviewer \thereviewer}}

